About Strongly Universal Cellular Automata

In this paper, we construct a strongly universal cellular automaton on the line with 11 states and the standard neighbourhood. We embed this construction into several tilings of the hyperbolic plane and of the hyperbolic 3D space giving rise to strongly universal cellular automata with 10 states.

==> eptcsdata.tex <==
\providecommand{\firstpage}{93}
\providecommand{\publicationstatus}{T. Neary and M. Cook (Eds.):\\
Machines, Computations and Universality (MCU 2013)\\
EPTCS 128, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.128.17}{10.4204/EPTCS.128.17}}

